Human101: Training 100+FPS Human Gaussians in 100s from 1 View

Reconstructing the human body from single-view videos plays a pivotal role in the virtual reality domain. One prevalent application scenario necessitates the rapid reconstruction of high-fidelity 3D digital humans while simultaneously ensuring real-time rendering and interaction. Existing methods often struggle to fulfill both requirements. In this paper, we introduce Human101, a novel framework adept at producing high-fidelity dynamic 3D human reconstructions from 1-view videos by training 3D Gaussians in 100 seconds and rendering in 100+ FPS. Our method leverages the strengths of 3D Gaussian Splatting, which provides an explicit and efficient representation of 3D humans. Standing apart from prior NeRF-based pipelines, Human101 ingeniously applies a Human-centric Forward Gaussian Animation method to deform the parameters of 3D Gaussians, thereby enhancing rendering speed (i.e., rendering 1024-resolution images at an impressive 60+ FPS and rendering 512-resolution images at 100+ FPS). Experimental results indicate that our approach substantially eclipses current methods, clocking up to a 10 times surge in frames per second and delivering comparable or superior rendering quality. Code and demos will be released at https://github.com/longxiang-ai/Human101.

==> figs/tex/sup_application.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/images/sup_application.png}
    \captionsetup{type=figure}
    % \vspace{-1.5em}
    \caption{\textbf{Application: track.} }
    \label{fig:appli_track}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/novel_view_1024.tex <==
\begin{table*}
\centering

\label{tab:novel_view_1024}
\begin{tabular}{|l|c|c|c|c|c|c|c|} \hline  
 & & \multicolumn{3}{|c|}{ZJU-MoCap}& \multicolumn{3}{|c|}{MonoCap}\\ \hline  

allhuman 1024 res& \textbf{Training Time} & \textbf{PSNR} & \textbf{SSIM} & \textbf{LPIPS*}  &\textbf{PSNR}  & \textbf{SSIM} &\textbf{LPIPS*}  
\\ \hline  

Ours & $\sim $ 5min& \textbf{32.65} & 0.979 & \textbf{16.13}  &\textbf{32.04}  & 0.977 &\textbf{16.13}  
\\ \hline  
 3D GS Original\cite{kerbl3Dgaussians}& & & & & & &
\\ \hline  

Instantnvr\cite{instant_nvr}& $\sim $ 5min & 31.36 & 0.979 & 26.03  &31.36  & 0.979 &26.03  
\\ \hline 
 Explicify\cite{zhang2023explicifying}& & & & & & &\\ \hline 

HumanNeRF\cite{weng_humannerf_2022_cvpr} & $\sim $ 10h & 31.12 & 0.977 & 22.80 &31.12  & 0.977 &22.80 
\\ \hline  

AS & $\sim $ 10h & 31.22 & \textbf{0.983} & 26.20 &31.22  & \textbf{0.983} &26.20 
\\ \hline  

NB\cite{peng2021neuralbody} & $\sim $ 10h & 29.50& 0.970& 28.32  &29.50 & 0.970&28.32  
\\ \hline  

AN\cite{peng2021animatablenerf} & $\sim $ 10h & 29.91 & 0.971 & 32.89  &29.91  & 0.971 &32.89  
\\ \hline  

% NHP & 10h pretrain + 1h finetune & 27.67 & 0.957 & 60.08  &27.67  & 0.957 &60.08  
% \\ \hline  

% PixelNeRF\cite{yu2021pixelnerf} & 10h pretrain + 1h finetune & 23.94 & 0.899 & 112.83  &23.94  & 0.899 &112.83  \\ \hline 


\end{tabular}
\caption{Comparison with state-of-the-art methods in 1024 $\times$  1024 resolution}
\end{table*}

==> tables/novel_view_512.tex <==

\begin{table}
\centering
\caption{Comparison with state-of-the-art methods in 512 $\times$  512 resolution, \textbf{novel view}}
\label{tab:novel_view_512}
\begin{tabular}{| l  |c|c|c|c|}
\hline
zjumocap& \textbf{Training Time　} & \textbf{PSNR} & \textbf{SSIM} & \textbf{LPIPS*} \\
\hline
Ours & 5min& \textbf{32.04} & 0.977 & \textbf{16.13} \\
 3D GS& 5min& & &\\
\hline
Instantnvr& 5min & & & \\
 InstantAvatar& 5min& 22.10& 0.901&132.5\\\hline
\hline
HumanNeRF & 10h & & & \\
\hline
AS & 10h & & & \\
\hline
NB & 10h & & & \\
\hline
AN & 10h & & & \\

\end{tabular}

\end{table}


\begin{table}
\centering
\caption{Comparison with state-of-the-art methods in 512 $\times$  512 resolution, \textbf{novel view}}
\label{tab:novel_view_512}
\begin{tabular}{| l  |c|c|c|c|}
\hline
monocap& \textbf{Training Time　} & \textbf{PSNR} & \textbf{SSIM} & \textbf{LPIPS*} \\
\hline
Ours & 5min& & & \\
 3D GS& 5min& & &\\
\hline
Instantnvr& 5min & & & \\
 InstantAvatar& 5min& & &\\\hline
\hline
HumanNeRF & 10h & & & \\
\hline
AS & 10h & & & \\
\hline
NB & 10h & & & \\
\hline
AN & 10h & & & \\

\end{tabular}

\end{table}


==> tables/test.tex <==
\begin{table}[htb]
    \centering
    \caption{Quantitative comparison of human reconstruction methods.}
    \label{tab:all_comparison}
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
    \rowcolor{gray!50}
    Method & Res. & Train & Publication & Year & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS* $\downarrow$ & FPS $\uparrow$ \\
    \hline
    \cellcolor{white}3D GS & 512 & $\sim$5min & SIGGRAPH & 23 & 26.57 & 0.935 & 71.7 & 28.47 \\
    \cellcolor{white}3D GS & 1024 & $\sim$5min & SIGGRAPH & 23 & 26.53 & 0.944 & 58.23 & 27.47 \\
    \addlinespace
    NeuralBody & 512 & $\sim$10h & CVPR & 21 & 29.03 & 0.964 & 42.47 & 3.5 \\
    % ... add other rows here
    \addlinespace
    Ours w/o SMPL Deformation & 512 & 100s & - & 23 & 28.70 & 0.964 & 41.61 & - \\
    % ... add other rows here
    \addlinespace
    \rowcolor{bestcolor}
    \textbf{Ours full} & 1024 & 5min & - & 23 & 32.18 & 0.977 & 21.32 & 666 \\
    \end{tabular}
\end{table}
